How Can Graph Neural Networks Help Document Retrieval: A Case Study on CORD19 with Concept Map Generation

Graph neural networks (GNNs), as a group of powerful tools for representation learning on irregular data, have manifested superiority in various downstream tasks. With unstructured texts represented as concept maps, GNNs can be exploited for tasks like document retrieval. Intrigued by how can GNNs help document retrieval, we conduct an empirical study on a large-scale multi-discipline dataset CORD-19. Results show that instead of the complex structure-oriented GNNs such as GINs and GATs, our proposed semantics-oriented graph functions achieve better and more stable performance based on the BM25 retrieved candidates. Our insights in this case study can serve as a guideline for future work to develop effective GNNs with appropriate semantics-oriented inductive biases for textual reasoning tasks like document retrieval and classification. All code for this case study is available at https://github.com/HennyJie/GNN-DocRetrieval.

==> old_sections/concept-map.tex <==
\section{Concept Map Construction and Utility Assessment}
\label{sec:map}

% \begin{table}[]
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% Pair Type & \bf \# Pairs & \bf Node CR & \bf Freq CR & \bf Edge CR & \bf TFIDF \\ \midrule
% Positive & 762,084  & 0.050 & 0.174 & 0.006 & 0.192        \\
% Contrary & 1,518,617 & 0.041 & 0.15 & 0.004 & 0.117        \\
% (t-score) & -  & 187.041 & 274.468 & 83.569 & 487.078      \\
% BM25 & 140,640 & 0.038 & 0.145 & 0.004 & 0.150  \\
% (t-score) & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% \caption{Concept Map Analysis}
% \label{tab:structure}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
% T-test & {\bf CV} & \bf Node CR & \bf Freq CR & \bf Edge CR & \bf TFIDF  \\ \midrule
% t-score & 1.645  & 187.041 & 274.468 & 83.569 & 487.078       \\
% \bottomrule
% \end{tabular}
% \caption{Significance Test}
% \label{tab:ttest}
% \end{table}
As shown in our toy example, effectively digging out the structured knowledge from unstructured texts can potentially provide clear inductive bias for downstream applications and support the interpretability of deep learning models. Here we devise a concept map construction pipeline and analyze its potential utility for document retrieval from both structural and semantic perspectives.

\header{Concept map construction.}
% We aim to distill structured information hidden under natural language sentences and represent it with a graph structure. In textual documents, entities and events often convey rich semantics, and thus containing significant fractions of the information. Although Name Enity Recognition (NER), open-IE and other off-the-shelf NLP tools have shown great ability in identifying such salient language units in documents, the performance of these tools in the emerging biomedical domain as we consider is limited due to the lack of training data \cite{wang2018comparative}. %Consequently, existing tools fail to identify enough mentions as entities, leading to insufficient nodes in the concept maps. 
% \hejie{Concept map construction from text has been studied extensively in literature \cite{tseng2007new, DBLP:journals/ce/ChenKWC08, DBLP:conf/softcom/ZubrinicOS15, DBLP:conf/nips/YangZSL019, DBLP:conf/wsdm/YangZWLKWX020, DBLP:journals/corr/abs-2101-11873}. We tried several different methods in preliminary studies and adopted the one producing the most informative graphs here.} Specifically, we identify noun phrases and verb phrases to reflect salient entities and events by applying the more primitive but reliable POS-tagging and constituency parsing~\cite{manning-etal-2014-stanford}. %, which are relatively more reliable and can extract sufficient phrases as node candidates.
% The identified phrases are simplified by removing articles (\textit{a, an, the}) and replacing with lemmas, and then merged by same mentions. Furthermore, to capture the interactions among extracted nodes \hejie{which compose the edges in graphs}, we follow the common practice in phrase graph construction \cite{mihalcea2004textrank} and use \hejie{fixed size sliding windows for edge construction, where the window size is selected through grid search}. 
Concept map construction, which aims to distill structured information hidden under natural language sentences and represent it with a graph structure, has been studied extensively in literature \cite{tseng2007new,DBLP:journals/ce/ChenKWC08,DBLP:conf/softcom/ZubrinicOS15,DBLP:conf/nips/YangZSL019,DBLP:conf/wsdm/YangZWLKWX020,DBLP:journals/corr/abs-2101-11873}. For this case study, we tried several different methods and adopted the one producing the most informative graphs. Since entities and events often convey rich semantics, they are widely used to represent core information of documents and compose concept maps \cite{christensen-etal-2013-towards,li-etal-2020-connecting,lu2021evaluation}. 
% Although existing name entity recognition (NER) and relation extraction (RE) techniques have shown great ability in identifying salient language units in documents, concept maps constructed from NER or RE often suffer from few nodes and sparse edges issues according to our pilot trials. 
According to our pilot trials, concept maps constructed from existing NER or RE tools often suffer from limited nodes and sparse edges.
Moreover, these techniques rely on significant amounts of training data and predefined entities and relation types, whose availability is limited in the emerging domain as we consider \cite{wang2018comparative}.

To deal with the lack of supervision in biomedical domain and increase node/edge coverage, in our practice, we identify noun phrases and verb phrases to reflect salient entities and events (which compose the nodes in graphs), by POS-tagging and constituency parsing \cite{manning-etal-2014-stanford}. Compared to concept maps derived from NER or RE, our graphs can better represent original documents by identifying more sufficient phrases as nodes and connecting them with denser edges, as pos-tagging and parsing are more robust to domain shift \cite{mcclosky2010automatic,yu2015domain}.
The identified phrases are filtered via removing articles (\textit{a, an, the}) and replacing lemmas, and then merged by the same mentions. Furthermore, to capture the interactions among extracted nodes (which compose the edges in graphs), we follow the common practice in phrase graph construction \cite{mihalcea2004textrank,rose2010automatic,krallinger2005sentence} using the sliding window technique to capture node co-occurrence. The window size is selected through grid search. To our knowledge, this pipeline represents the most ideal way to construct concept maps in an emerging domain as we consider in this study.

\header{Utility assessment.}
To empirically manifest the potential utility of our constructed concept maps for document retrieval, we conduct several assessments from both semantic and structural perspectives. 

Based on the ground-truth relevance labels, we construct a Pos-Pos pair with two documents that are both relevant to a query; similarly, we construct a Pos-Neg pair with one relevant document and one irrelevant. Moreover, we construct a Pos-BM pair with one relevant document and one document ranked top-20 by BM25.
% given a query considering NDCG@20 is the most important evaluation metric.
All pairs are constructed and analyzed exhaustively over all queries. 
%All possible combinations over pairs are extracted from the full version set of accumulated judgement released after all rounds. Four different types of structure and semantic metrics are evaluated, including:
The concept map similarity between the pairs of documents is compared via four types of measures including
\begin{list}{$\bullet$}{\leftmargin=1em \itemindent=0em}
    \item \textbf{NCR}: node coincidence rate between $G_i$ and $G_j$.
        \begin{equation}
			CR_{i, j}^V = \frac{\lvert V_i \cap V_j \rvert}{\lvert V_i \cup V_j \rvert}.
		\end{equation}
    % \item \textbf{NCR+}: to make the setting closer to document retrieval, we further weight NCR by the TF-IDF scores \cite{baeza1999modern} of each node (word or phrase in documents).
    \item \textbf{NCR+}: NCR weighted by the TF-IDF scores \cite{baeza1999modern} of each node (word or phrase in documents), which makes the setting closer to document retrieval.
    \item \textbf{ECR}: edge coincidence rate between $G_i$ and $G_j$, where an edge is coincident when the two ends of it are contained in both graphs.
    \item \textbf{ECR+}: ECR weighted by the TF-IDF scores of nodes on both ends of the edges.
\end{list}

The purpose is to validate that information in the constructed concept maps can indicate query-document relevance, which is true if the Pos-Pos pairs of documents are more similar to each other compared with the Pos-Neg pairs; moreover, the concept maps can provide additional signals compared to traditional IR methods: if the Pos-BM pairs are not similar enough compared with the Pos-Pos pairs, or even not more similar compared with the Pos-Neg pairs.

As shown in Table \ref{tab:structure}, the results uphold our assumption towards the utility of concept maps in document retrieval, where the Pos-Neg pairs are less similar compared with the Pos-Pos pairs regarding all measures. Moreover, the Pos-BM pairs are not close to the Pos-Pos pairs and even further away than Pos-Neg ones. This is indeed not too surprising because the ``irrelevant'' documents labeled by experts are not selected randomly, but rather hard negative ones from previous competition submissions. %For example, given a query "violent crime in society", a document with seemingly relevant concepts like "mental health, violence, anxiety" is judged as negative, since it actually talks about what challenges pandemic could bring to doctors. 
Such results clearly indicate a large room for improving traditional IR with concept maps. 

To further analyze the significance of the results, we perform student's t-Test over the three groups of samples \cite{hogg2005introduction}. Given the number of samples, the critical value (\textit{CV}) for 95\% confidence between Pos-Pos and Pos-Neg is 1.6440, whereas the (\textit{CV}) between Pos-Pos and Pos-BM is 1.6450. The actual \textit{t-scores} shown in Table \ref{tab:structure} strongly support the significance of differences between the Pos-Pos and Pos-Neg pairs, as well as the Pos-Pos and Pos-BM pairs.

\begin{table}[t]
\centering
\caption{Concept map utility analysis results.}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
Pair Type & \bf \# Pairs & \bf NCR & \bf NCR+ & \bf ECR & \bf ECR+ \\ \midrule
Pos-Pos & 762,084  & 0.0496 & 0.1919 & 0.0060 &  0.0078       \\
Pos-Neg & 1,518,617 & 0.0412 & 0.1175 & 0.0039 &  0.0052       \\
\rowcolor{gray!20} (\textit{t-score}) & -  & (\textit{187.041}) & (\textit{487.078}) & (\textit{83.569}) &  (\textit{105.034})    \\
Pos-BM & 140,640 & 0.0380 & 0.1498 & 0.0037 & 0.0043 \\
\rowcolor{gray!20} (\textit{t-score}) & - & (\textit{126.977}) & (\textit{108.808}) & (\textit{35.870})  & (\textit{56.981}) \\
\bottomrule
\end{tabular}
}
\label{tab:structure}
\end{table}

%of d compared with the critical value (\textbf {CV}) calculated using the degrees of freedom and the percent point function (PPF) for a given significance level 0.05 (95\% confidence), the absolute value of each test statistics is much higher, especially, the TFIDF similarity reaching up to 480. The statistic values interpret we strongly reject the null hypothesis that the means of positive pairs an contrary pairs are equal. This implies that documents relevant to the same query constantly contains more overlap information than those does not, which verifies the effectiveness and discrimination degree of our constructed concept map from both structural and semantic perspectives. 

==> old_sections/discussion.tex <==
\section{Conclusion and Future Work}
\label{sec:insight}

%\carl{table: powerful gnns much worse than simplified graph function, because too complex, irrelevant bias, hard to train, easy to overfit; while simplified models proper for graph modeling, focusing on simple interactions. In order to further justify such insights, we conduct... }

% \begin{figure}[!]
% \hspace{-5mm}
% \begin{subfigure}[b]{0.5\linewidth}
% \includegraphics[width=\linewidth]{figures/consistency_ndcg20.pdf}
% \vspace{-0.5cm}
% \caption{Consistency assessment}
% \label{fig:consis_ndcg20}
% \end{subfigure}
% \hspace*{\fill}
% \begin{subfigure}[b]{0.5\linewidth}
% \includegraphics[width=\linewidth]{figures/training_curves.pdf}
% \vspace{-0.5cm}
% \caption{Testing curves}
% \label{fig:train_curve_ndcg20}
% \end{subfigure}
% \caption{In-depth analysis of different graph models.}
% \label{fig:analysis}
% \end{figure}

\begin{figure}[t]
	\centering
	\subfloat[Consistency assessment]{
	    \centering
		\includegraphics[width=0.4\linewidth]{figures/consistency_ndcg20.pdf}
		\label{fig:consis_ndcg20}
	}
	\subfloat[Testing curves]{
	    \centering
		\includegraphics[width=0.4\linewidth]{figures/training_curves.pdf}
		\label{fig:train_curve_ndcg20}
	}
	\caption{In-depth analysis of different graph models.}
	\label{fig:analysis}
\end{figure}

As revealed in Table \ref{tab:perform}, existing powerful GNNs perform much worse than the proposed simplified graph functions and even mess up the results from the initial ranking phrase. We believe such performance loss is due to their over-modeling of the concept map structures, which makes them prone to overfitting and hard to generalize.  To be specific, the major inductive bias on complex structures makes limited contribution to the document retrieval task and is easily misled by noises. 

To further justify our conjectures, we examine the performance of different models across multiple runs-- as shown in Fig.\ref{fig:analysis} (a), the results of GIN and GAT are less consistent, indicating the difficulty in training over-complex models. Moreover, from the testing curves of different models during training-- as shown in Fig.\ref{fig:analysis} (b), we find GIN can hardly improve during training, possibly due to its irrelevant inductive bias towards complex graph structures and less effective modeling of simple semantics, whereas GAT is fluctuating and clearly suffering from overfitting.

In contrast, the proposed simplified graph functions perform much more stable in Fig.\ref{fig:analysis} (a), and improve more efficiently during training in Fig.\ref{fig:analysis} (b), demonstrating their abilities to effectively model the concepts and simple interactions important for the retrieval task. Among the three functions, E-Pool and RW-Pool are consistently better than N-Pool, revealing the utility of simple graph structures. Moreover, RW-Pool converges slower but achieves slightly better and more stable results in the end, indicating the potential utility of higher-order interactions. 

In the future, more datasets from various domains can also be included for exploration. Our study can serve as a guideline for designing more novel GNNs that are both more powerful while less prone to overfitting for semantic reasoning, thus benefiting document retrieval and other concept map related tasks.

%While, focusing on simple interactions, simplified models proper for graph modeling by taking advantage from graph structure while preserving the original semantic information. Among the three simplified graph models, E-Pool and RW-Pool exceed N-Pool, indicating simple interaction hidden in the structure secure ampler covered knowledge than individual nodes. In order to further justify such insights, we conduct extended experiments for interpretation.

%Since the performance results in Table \ref{tab:perform} is averaged among multiple runs, while except for the numeral difference on averaged values, models may also vary on their consistency, meaning how likely the results can be repeated with more runs. To further examine how consistent the discernibility of different models hold, we explicitly show the results from multiple runs in Figure \ref{fig:consis_ndcg20}. It is clear that N-Pool, E-Pool and RW-Pool possess much more stable performance than GNNs across different runs. This promotes the rationality of our conclusion that simplified permutation invariant functions perform better than powerful GNNs on reranking.

%To compare the convergence speed, we plot the training curve with the increase of  training epoch numbers in Figure \ref{fig:train_curve_ndcg20}, where the highlight curves depicts the average of five different runs and the light shadow represents the range of fluctuation after specific epochs for different runs. As is present, GIN rarely make any improvement during the process of training, indicating that GIN is not able to capture meaningful inductive bias and could even be suppressed with more training epochs due to over-fitting. Although GAT shows an fluctuant improving tendency, many more epochs might be needed for potential improvements, while its consistency is much worse compared with simplified functions in general. Among three simplified graph models, E-Pool and RW-Pool privilege than N-Pool after more training, which indicates that simple interaction assist in the graph structures than independent individuals. RE-Pool achieves the best performance, though it converge slower than E-Pool due to its higher computation complexity and the generalization with dynamic random walks.

%This case study on GNNs representation ability for TREC-COVID inspires us on the future directions for utilizing structured data in information retrieval task. An interesting future work is to design more efficient GNN models that can digest simple interactions while keep the original semantic information as much as possible while aggregation. Another interesting research venue is to generalize or quantify how much the structured information concealed underneath text can benefit and balance the structural and semantic leverage for different types of task. 

==> old_sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

%\carl{para 1: GNNs are powerful, concept maps are potentially helpful to make GNNs useful for document retrieval, toy example of how concept maps + GNNs might advance document retrieval}\\
%\carl{para 2: \textbf{Contribution 1:} construction and preliminary analysis on the utility of concept maps (refer to section 2 Concept Map Construction and Analysis)}\\
%\carl{para 3: \textbf{Contribution 2:} applying state-of-the-art GNNs for document re-ranking based on BM25 under the help of concept maps (refer to section 3 SOTA GNNs for Document Retrieval)}\\
%\carl{para 4: \textbf{Contribution 3:} designing simplified permutation-invariant functions on graphs for document retrieval (refer to section 4 Simplified Permutation-Invariant Graph Functions)}\\
%\carl{para 5: \textbf{Contribution 4:} insightful analysis and discussion over our empirical findings (refer to section 5 Insightful Analysis and Discussions)}\\
% \carl{So we have 4 sections besides introduction, each on one contribution. We do not need a separate experiments section, and instead we can put experimental results directly in section 2-4, and even some specific ones in section 5. Depending on the space, we can have or not have a related work section (it is not a must in short papers). Try to be concise in each section (everywhere), because you will extremely easily run over length for a 4-page paper.}

Concept map, which models text as a graph whose vertices represent words/phrases and edges represent their relations, has been studied to improve information retrieval tasks for a long time \cite{DBLP:conf/cscwd/ZhangWXP18,DBLP:journals/prl/FarhiB18,DBLP:journals/ir/BlancoL12,DBLP:conf/ecir/Kamphuis20}. Recently, graph neural networks (GNNs) attract tremendous attention from researchers across various domains due to their superior power established both in theory and through experiments \cite{kipf2016semi,hamilton2017inductive,velivckovic2018graph,ying2018hierarchical,liu2019geniepath,chen2018fastgcn}. Empowered by the structured document representation of concept maps, it is intriguing to apply powerful GNNs for text mining tasks such as document classification \cite{DBLP:conf/sigir/YangZWL020} and retrieval \cite{DBLP:journals/corr/abs-2101-11873}. Take Figure \ref{fig:toy-example} as an example. Towards the query  about ``violent crimes in society'', based on the concept map representation, a proper GNN might be able to highlight important query-relevant concept of ``crime'' and its connection to ``robbery'', ``citizen'' and ``challenge'' from a document, thus ranking it as highly relevant. On the other hand, for another document about
precaution, the GNN can capture concepts like ``hand washing'', ``n95 mask'' and ``distancing'', together with their connections to ``prevention'', thus ranking it as not so relevant.

\header{Present work.} In this work, we conduct a case study to explore the power of GNNs for document retrieval under the help of concept maps. The core contributions of this paper are four-fold:
\begin{list}{$\bullet$}{\leftmargin=1em \itemindent=0em}
    \item We construct concept maps from full-text documents based on various techniques and perform preliminary analyses on the potential utility of them towards document retrieval (Section \ref{sec:map}).
    \item We adapt and evaluate state-of-the-art (SOTA) GNNs on the structured document representations of concept maps for document re-ranking based on the BM25 baseline (Section \ref{sec:sota}).
    \item Reflecting on the limited performance of SOTA GNNs, we design and evaluate several simplified permutation-invariant graph functions in the same re-ranking settings (Section \ref{sec:simple}).
    \item We provide further analysis and insights towards the limited performance of SOTA GNNs and surprisingly good performance of simplified graph functions, and conclude with potential future directions inspired by this study, with the hope to prompt more discussions on emerging areas such as IR with GNNs on concept maps (Section \ref{sec:insight}). 
\end{list}

==> old_sections/setup.tex <==
\section{Dataset and Experimental Setup}
\label{sec:setup}

\begin{figure*}[]
    \centering
    \includegraphics[width=\linewidth]{figures/toy-example.pdf}
    \caption{Toy example of concept maps and GNN-based document re-ranking. %\carl{possible to give more detailed narrations here later if space permits (eg., what is alpha, which concepts/structures are highlighted for relevance modeling).}
    }
    \label{fig:toy-example}
\end{figure*}

\header{Dataset.}
In this study, we focus on the dataset from TREC-COVID\footnote{\label{ft:trec-covid}https://ir.nist.gov/covidSubmit/}, a document retrieval challenge held in response to the pandemic. % and facilitating reliable information retrieval on virus and it impact searching for researchers, clinicians and policy makers. 
The raw data include three parts: a growing  corpus CORD-19\footnote{\label{ft:cord19}https://github.com/allenai/cord19} \cite{wang-etal-2020-cord} in broad  research areas, a set of pandemic-related queries that interest people, and dynamically released query-document relevance labels. 
For each query, a set of positive documents and a set of negative ones are provided as ground-truth. We take the round 5 dataset from the challenge, which includes 192,509 documents, 50 queries and 46,167 judgements in total.

% \header{Problem definition.} As a common practice, the large-scale document retrieval task can be solved in a two-step procedure, i.e., unsupervised candidate retrieval and supervised candidate re-ranking \cite{liu2011learning,dang2013two,nogueira2019passage}. Specifically in our setting, the initial retrieval on the whole corpus with full texts is performed through BM25 implemented based on Apache Lucene\footnote{https://lucene.apache.org/}, which is a a traditional yet powerful probabilistic retrieval framework used widely by search engines, also constitutes our baseline model. Then, based on the initial ranking list, we further conduct re-ranking on the top 100 documents using different GNN models, focusing on the potentially important structural information underlying the textual data. Then, based on the initial ranking list, we further conduct re-ranking on the top 100 documents using different GNN models, focusing on the potentially important structural information underlying the textual data. 


\header{Experimental settings.} As a common practice, the large-scale document retrieval task can be solved in a two-step procedure, i.e., unsupervised candidate retrieval and supervised candidate re-ranking \cite{liu2011learning,dang2013two,nogueira2019passage}. Specifically in our settings, the initial retrieval is performed on the whole corpus with full texts through BM25 based on Apache Lucene \cite {Robertson1994OkapiAT}, which is a traditional yet powerful retrieval method widely used in search engines. In this paper, we focus on exploring whether GNNs can improve on top of the BM25 initial retrieval results under the help of concept maps. % in stead of beating the most advanced neural IR models. 
Therefore, BM25 serves two roles in our experiments, the method to produce an initial candidate list and a baseline for GNN-based re-ranking.


\header{GNN for document re-ranking.}
Based on the initial candidates of each query from BM25, we further conduct re-ranking on the top 100 documents using different GNN models, to explore the potential of structural information underlying the textual data. The toy example in Figure \ref{fig:toy-example} presents the process of GNN-based document re-ranking.

A concept map \(G = \{V, E\}\) is first constructed for each document, where \(V\) and \(E\) denote the node set and link set, respectively. Each node \(v_i \in V\) is a concept (usually a word or phrase) in the document,  associated with a frequency $f_i$ and an initial feature vector $\bm a_i$ computed from BioWordVec \cite{zhang2019biowordvec}, which provides pre-trained word embeddings in biomedical contexts. The links in \(E\) denote the interaction between concepts. Higher-order interactions can then be captured by random walks $P$ on $G$. 

We then aim to encode both structural and semantic information in the concept maps by node representations \(\bm{h}_i \in \mathbb{R}^{d}\) learned by GNNs, where \(d \ll |V|\) is the embedding dimension. The graph-level embedding \(\bm{h}_G \in \mathbb{R}^{d}\) is summarized over all nodes with a global read-out function.  %\textsuperscript{\ref{foot:biosentvec}}. 
We adopt the widely-used triplet loss in retrieval tasks \cite {DBLP:conf/iccv/ManmathaWSK17,DBLP:conf/kdd/YingHCEHL18,DBLP:conf/kdd/YangPZP0RL20}, for the training of GNNs here, i.e.,
\begin{align}
L(Q, G_p, G_n)=\max \left\{ S\left(G_n \mid Q \right) - S\left(G_p \mid Q \right)+\textit{margin}, 0\right\}.
\label{eq:triplet}
\end{align}
Given a query \(Q\), the final relevance score \(S(G\mid Q)\) in Eq.~\eqref{eq:triplet} is computed as the cosine similarity between the graph representation $\bm h_G$ and the query representation $\bm h_Q$ from BioSentVec \cite{chen2019biosentvec}.
%$$S \left(G \mid Q \right) = \frac{\bm{h}_G \cdot \bm{h}_Q}{\|\bm{h}_G \|\|\bm{h}_Q\|}$$
During the training, the embeddings of documents relevant to a given query are pulled towards the query representation; on the contrary, those irrelevant ones are pushed away. In the testing phrase, documents are then re-ranked according to their score $ S\left(G \mid Q \right)$.

\header{Evaluation metrics.}
The evaluation metrics used in this study are mainly adopted from those used for the competition, among which NDCG@20 is used for ranking on the leader board. Besides NDCG@\textit K (\textit K=10, 20), we also use Precision@\textit K (\textit K=10, 20) and Recall@\textit K (\textit K=10, 20), which are both standard evaluation metrics for document retrieval. We focus on relatively small $K$ values, since users are more likely to only care about the top retrieved results. 

==> old_sections/simple-gnn.tex <==
\section{Simplified Permutation-Invariant Graph Functions}
\label{sec:simple}

% \begin{table*}[ht]
%  \centering
%  \begin{tabular}{lcccccccccccccc}
%  \hline
% \multirow{2}{*}{Metrics}&\multicolumn{2}{c}{\bf Baseline}&\multicolumn{4}{c}{\bf Node Pooling}&\multicolumn{4}{c}{\bf Edge Pooling} &\multicolumn{4}{c}{\bf Path Pooling}\\
% \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11} \cmidrule(lr){12-15}
% &{\it anserini } & \it{BM25} & \it{mean} &\it {sum} &\it{max} &\it{tfidf} & \it{mean} & \it{sum} & \it{max} & \it{tfidf} & \it{mean} & \it{sum} & \it{max} & \it{tfidf}\\
% \hline
% P@10 & 0.5400 & 0.5520 & 0.5700 & \bf 0.59\40 & 0.5520 & \bf 0.5920 & \bf 0.6020 & \bf 0.6160 & 0.5420 & \bf 0.6320 & \bf 0.6120 & \bf 0.6000 & 0.5820 & \bf 0.5840 \\
% P@20 & 0.4960 & 0.4900 & 0.5200 & \bf 0.5420 & 0.4880 & \bf 0.5440 & \bf 0.5410 & \bf 0.5440 & 0.4830 & \bf 0.5480 & \bf 0.5450 & \bf 0.5550 & 0.5070 & \bf 0.5420 \\
% recall@20 & 0.0225 & 0.0239 & 0.0238 & \bf 0.0255 & 0.0226 & \bf 0.0253 & \bf 0.0251 & \bf 0.0257 & 0.0221 & \bf 0.0255 & \bf 0.0254 & \bf 0.0261 & 0.0240 & \bf 0.0254 \\
% recall@40 & 0.0401 & 0.0401 & 0.0416 & \bf 0.0424 & 0.0388 & \bf 0.0422 & \bf 0.0429 & \bf 0.0436 & 0.0389 & \bf 0.0430 & \bf 0.0432 & \bf 0.0428 & 0.0410 & \bf 0.0418 \\
% ndcg@10 & 0.4709 & 0.5137 & 0.5471 & \bf 0.5551 & 0.5199 & \bf 0.5727 & \bf 0.5776 & \bf 0.5949 & 0.5237 & \bf 0.5934 & \bf 0.5869 & \bf 0.5786 & 0.5475 & \bf 0.5588 \\
% ndcg@20 & 0.4382 & 0.4591 & 0.4995 & \bf 0.5075 & 0.4651 & \bf 0.5250 & \bf 0.5224 & \bf 0.5284 & 0.4696 & \bf 0.5280 & \bf 0.5239 & \bf 0.5294 & 0.4897 & \bf 0.5181\\
% \hline
% \end{tabular}
% \caption{\label{tab:simplified}\small Rerank performance of Simplified Functions on different metrics}
% \end{table*}

The limited performance of SOTA GNNs on document re-ranking motivates us to reflect on the gap between current GNNs and the characteristics of document retrieval task. How to effectively distinguish relevant and irrelevant documents based on the semantic units in a graph structure needs to be re-examined.
%with the structural information underneath the graph along with the semantics and linguistics knowledge on the surface should be further examined in terms of document retrieval task.

In particular, although GIN is the most appropriate GNN for learning graph-level representations, its power mainly stems from the 1-WL test for graph isomorphism, which exhaustively tries to capture possibly complex graph structures so as to differentiate non-isomorphic graphs. However, in our setting, the exact structures of concept interactions may be less important for distinguishing the semantic relevance of documents. Instead, the concept-wise semantics organized by simple graph structures, such as the concepts themselves (e.g., ``robbery'' in Figure \ref{fig:toy-example}) and pairs of concepts (e.g., ``robbery'' and ``crime''), might be more useful. This motivates us to design simplified graph models easier to train and generalize.
% To do. Add theoretical basis.
%Recently, the Weisfeiler-Lehman (WL) test has been used to evaluate the expressive power of GNNs. WL test is a algorithm used to test graph isomorphism. Given a colored graph $G=(V, E, d)$ and a set of color $\Sigma$, where $|V|=n$ is the vertex set, then $d: V \rightarrow \Sigma$ defines color mappings that implies the color attached to each vertex. We call two graphs $G, G^{\prime}$ isomorphic if a color preserving bijection $\phi: V \rightarrow V^{\prime}$ exists. \(k\)-WL test the isomorphism of two graphs by first constructing a coloring of \(k\)-tuple of vertices, that is $c: V^{k} \rightarrow \Sigma$, and then comparing the colors histograms produced by \(k\)-WL algorithms \cite{NEURIPS2019_bb04af0f}. 

We again reflect on the properties of existing GNNs. We find that, besides various neighborhood transformations and propagation functions, existing GNNs mostly follow a \textit{message passing} mechanism on graphs \cite{gilmer2017neural}, which is essentially \textit{permutation invariant} \cite{maron2019universality,maron2018invariant,keriven2019universal}. That is, the results of GNNs are not influenced by the various possible orders of nodes or links in the graph. Following this insight, we propose the following series of simplified permutation-invariant graph functions, which inherit the graph-specific inductive bias of existing GNNs, while focusing on the basic semantic units and their simpler interactions in concept maps.

%Permutation invariance is a fundamental inductive bias of graph structured data, which means that the permutation of the nodes of the input graph does not affect the output. A family of permutation-invariant deep neural network models for graph have been proposed. The universality of invariant networks is studied for $k$-order graph networks by Maron et al. (2019a) \cite{maron2019universality}, where \(k\)-order networks are further proved to be able to distinguish between non-isomorphic graphs as good as the \(k\)-WL tests by \cite{NEURIPS2019_bb04af0f}. Specifically, given two graphs $G=(V, E, d), G^{\prime}=\left(V^{\prime}, E^{\prime}, d^{\prime}\right)$ that can be distinguished by the $k$-WL graph isomorphism test, there exists a $k$-order invariant network $F$ so that $F(G) \neq F\left(G^{\prime}\right) .$ On the other direction for every two isomorphic graphs $G \cong G^{\prime}$ and $k$-order permutation invariant network $F, F(G)=F\left(G^{\prime}\right)$.

%Inspired by the theorem about the expressive power of permutation invariant functions on graph data structure above, we apply three simplified permutation invariant functions with different \(k\)-order of on our undirected concept map, where \(k=1, 2, 3+\) corresponds to node pooling, edge pooling, and path pooling respectively.

\begin{list}{$\bullet$}{\leftmargin=1em \itemindent=0em}
\item \textbf{N-Pool}: independently process each single \textit{Node} in the concept map by multi-layer perceptions and then apply read-out to aggregate all node embeddings into the graph embedding, i.e., %then project the representation of each node to the feature space of the query. %Graph-level representation are summarized through different readout functions, including sum, mean, max and TFIDF weights. 
\begin{equation}
\bm h_{G}=\operatorname{READOUT}\Big( \{\operatorname{MLP}(\bm a_{i}) \mid v_i \in V \}\Big).
\end{equation}

\item \textbf{E-Pool}: for each \textit{Edge} in the concept map, further concatenate the projected node embedding on its two ends to encode first-order interactions, and apply read-out to aggregate all edge embeddings into the graph embedding, i.e., 

% \begin{scriptsize} 
% \begin{equation} 
% h_{G}=\operatorname{CONCAT}\left(\operatorname{READOUT}\left(\left\{cat \left( h_{i}^{(k)}, h_{j}^{(k)} \right) \mid (i,j) \in E\right\}\right) \mid k=0,1, \ldots, K\right).
% \end{equation} 
% \end{scriptsize}
\begin{equation}
\bm h_{G}=\operatorname{READOUT}\Big(\left\{cat \left( \operatorname{MLP}(\bm a_{i}), \operatorname{MLP}(\bm a_{j}) \right) \mid e_{ij} \in E\right\}\Big).
\end{equation}

\item \textbf{RW-Pool}: sample \textit{Random Walks} to encode higher-order interactions among concepts ($len=2,3,4$ in our experiments); for each random walk, the embedding is computed from the sum of all node embeddings on it, and read-out is applied to aggregate all random walk embeddings into the graph embedding, i.e.,
% \begin{tiny} 
% \begin{equation} 
% h_{G}=\operatorname{CONCAT}\left(\operatorname{READOUT}\left(\left\{sum \left( h_{p_1}^{(k)}, h_{p_2}^{(k)},\ldots, h_{p_m}^{(k)} \right) \mid (p_1, p_2, \ldots, p_m) \in P\right\}\right) \mid k=0,1, \ldots, K\right).
% \end{equation} 
% \end{tiny}
\begin{equation}
\begin{aligned}
\bm h_{G}=\operatorname{READOUT}\Big( 
\{ sum \left( \operatorname{MLP}(\bm a_1), \operatorname{MLP}(\bm a_2), \ldots, \operatorname{MLP}(\bm a_m) \right ) \\
\mid (v_1, v_2, \ldots, v_m) \in P \}\Big).
% \bm h_{G}=\operatorname{READOUT}\left(\left\{sum \left( h_{p_1}^{(k)}, h_{p_2}^{(k)},\ldots, h_{p_m}^{(k)} \right) \mid (p_1, p_2, \ldots, p_m) \in P\right\}\right) 
\end{aligned}
\end{equation}
\end{list}

By design, all three graph functions are permutation-invariant and easy to compute, and they capture different levels of simple interactions among concepts in the graph. Other types of such simplified functions can be designed, such as longer random walk and motif based-pooling. We leave the exploration of them as future work.

\header{Results.} The performance of our simplified permutation-invariant graph functions are presented in the last three rows of Table \ref{tab:perform}. Here we focus on the performance difference between the simplified permutation-invariant functions and complicated GNNs. Although we do not directly compare with the heavier language models such as those based on BERT \cite{DBLP:conf/naacl/DevlinCLT19,DBLP:conf/emnlp/YilmazWYZL19,DBLP:journals/corr/abs-2007-12603} and learning to rank \cite{DBLP:conf/icml/BurgesSRLDHH05,DBLP:journals/ir/WuBSG10}, the absolute performances are benchmarked with strong baselines such as Anserini and BM25. Impressively, three proposed graph functions all yield significant and consistent improvements over both baselines and SOTA GNN models. Notably, E-Pool and RW-Pool can improve the document ranking from the initial ranking of BM25 by 11.4\% and 12.0\% on NDCG@20, respectively.
Such results support our insights and demonstrate the potential of further designing concept map oriented GNNs for document-level tasks like classification, retrieval, and certain semantic reasoning. 

==> old_sections/sota-gnn.tex <==
\section{SOTA GNNs for Document Retrieval}
\label{sec:sota}

% \begin{table*}[ht]
%  \centering
%  \begin{tabular}{lcccccccccc}
%  \hline
% \multirow{2}{*}{Metrics}&\multicolumn{2}{c}{\bf Baseline}&\multicolumn{4}{c}{\bf GIN}&\multicolumn{4}{c}{\bf GAT}\\
% \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}
% &{\it anserini } & \it{BM25} & \it{mean} &\it {sum} &\it{max} &\it{tfidf} & \it{mean} & \it{sum} & \it{max} & \it{tfidf}\\
% \hline
% P@10 & 0.5400 & 0.5520 & 0.4020 & 0.3520 & 0.3780 & 0.3320 & \bf 0.5920 & \bf 0.5980 & 0.5100 &	\bf 0.5820 \\
% P@20 & 0.4960 & 0.4900 & 0.3840 & 0.3320 & 0.3750 & 0.3070 & \bf 0.5310 & \bf 0.5500 & 0.4600  & \bf 0.5330 \\
% recall@20 & 0.0225 & 0.0239 & 0.0161 & 0.0151 & 0.0164 & 0.0147 & \bf 0.0252 & \bf 0.0259 & 0.0209 & \bf 0.0249 \\
% recall@40 & 0.0401 & 0.0401 & 0.0310 & 0.0298 & 0.0299 & 0.0287 & \bf 0.0430 & \bf 0.0428 & 0.0366 & \bf 0.0435\\
% ndcg@10 & 0.4709 & 0.5137 & 0.3550 & 0.3081 & 0.3223 & 0.2926 & \bf 0.5659 & \bf 0.5638 & 0.4700 & \bf 0.5494 \\
% ndcg@20 & 0.4382 & 0.4591 & 0.3431 & 0.2917 & 0.3199 & 0.2767 & \bf 0.5101 & \bf 0.5192 & 0.4281 & \bf 0.5092 \\
% \hline
% \end{tabular}
% \caption{\label{tab:gnns}\small Rerank performance of SOTA GNNs on different metrics}
% \end{table*}

With the structured document representation of concept maps, GNNs can be applied to this task following a neural message passing scheme \cite{gilmer2017neural,verma2019stability}, where node representation is updated through recursive transformation and aggregation from its neighbors. Many GNN variants with different neighborhood transformation and aggregation functions have been proposed. Here we treat document concept maps as individual graphs and adopt two SOTA GNNs for graph-level representation learning towards document retrieval.

% \header{Graph isomorphism network (GIN).} GIN is a simple yet powerful class of GNNs with equivalent discriminative and representational power as the 1-Weisfeiler-Lehman (1-WL) test, which is the upper bound for graph-level GNN representation capacity proved in \cite{xu2018powerful}.
\header{Graph isomorphism network (GIN).} GIN \cite{xu2018powerful} is a simple yet arguably the most powerful GNN for graph-level representation learning as proved in \cite{xu2018powerful}. GIN updates the representation of node \(v_i\) in the \(k\)-th layer as
\begin{equation}
\bm h_{i}^{(k)}=\mathrm{MLP}^{(k)}\left(\left(1+\epsilon^{(k)}\right) \cdot \bm h_{i}^{(k-1)}+\sum_{j \in \mathcal{N}(i)} \bm h_{j}^{(k-1)}\right), 
\label{eq:gin}
\end{equation}
where \(\epsilon^{(k)}\) can be either a learnable parameter or a fixed scalar and \(\mathcal{N}(i)\) denotes all neighboring nodes of node \(v_i\). The graph-level representation is then obtained by concatenating the read-out, i.e. the mapping from the representations of all nodes in the graph to a single representation of the whole graph as

\begin{equation}\nonumber
\bm h_{G}=\operatorname{CONCAT}\left(\operatorname{READOUT}\left(\{\bm h_{i}^{(k)} \mid v_i \in G\}\right) \mid k=0,1, \ldots, K\right).
\end{equation}

% \header{Graph attention network (GAT)}. GAT employs an attention mechanism to assign different weights for different nodes in a neighborhood. It computes a weighting factor \(\alpha_{ij}\) of neighboring node \(v_j\) to center node \(v_i\) with pair-wise attention as $a: \mathbb{R}^{D} \times \mathbb{R}^{D} \rightarrow \mathbb{R}$. \(\alpha_{ij}\) normalizes the coefficients \(e_{ij}\) across all neighbors based on their representation at each GAT layer as
% $$
% \alpha_{i j}=\frac{\exp \left(e_{i j}\right)}{\sum_{k \in \mathcal{N}_{i}} \exp \left(e_{i k}\right)},
% $$
% where $e_{i j}=a\left(\bm{h}_{i}, \bm{h}_{j}\right)$, $v_j\in \mathcal{N}_i$. We combine the attention mechanism in GAT with GIN by replacing Eq.~\eqref{eq:gin} with
% \begin{equation}
% \bm h_{i}^{(k)}=\mathrm{MLP}^{(k)}\left(\left(1+\epsilon^{(k)}\right) \cdot \bm h_{i}^{(k-1)}+\sum_{j \in \mathcal{N}(i)} \alpha_{i j} \cdot  \bm h_{j}^{(k-1)}\right), 
% \label{eq:gat}
% \end{equation}
% and refer to this improved GIN with attention as GAT in the rest of this work.

\header{Graph attention network (GAT)}. GAT \cite{velivckovic2018graph} employs an attention mechanism to assign different weights for different neighbors in each graph convolution layer. It computes a weighting factor \(\alpha_{ij}\) as
$$
\alpha_{i j}=\frac{\exp \left(m\left(\bm{h}_{i}, \bm{h}_{j}\right)\right)}{\sum_{v_k \in \mathcal{N}_{i}} \exp \left(m\left(\bm{h}_{i}, \bm{h}_{k}\right)\right)},
$$
where $m: \mathbb{R}^{d} \times \mathbb{R}^{d} \rightarrow \mathbb{R}$ is the learnable attention function. We combine the attention mechanism in GAT with GIN by replacing Eq.~\eqref{eq:gin} with
\begin{equation}
\bm h_{i}^{(k)}=\mathrm{MLP}^{(k)}\left(\left(1+\epsilon^{(k)}\right) \cdot \bm h_{i}^{(k-1)}+\sum_{j \in \mathcal{N}(i)} \alpha_{i j} \cdot  \bm h_{j}^{(k-1)}\right), 
\label{eq:gat}
\end{equation}
and refer to this improved GIN with attention as GAT in the rest of this work.

\header{Results.} The performance of the two SOTA GNNs are shown in the two middle rows of Table \ref{tab:perform}.
Besides BM25 for the initial retrieval, we also include the most updated performance from Anserini\footnote{https://git.uwaterloo.ca/jimmylin/covidex-trec-covid-runs/-/tree/master/round5} under the same settings as ours, which is a strong baseline recognized by the competition organizers and the TREC community. Different read-out functions are experimented on both GIN and GAT, including mean, sum, max and our designed TF-IDF (i.e., use the TF-IDF scores to weight the nodes before sum pooling), and the averaged results of multiple runs under the best settings are reported. 
% The mean, sum and max are traditional read-out functions and TF-IDF is our novel design for the document retrieval task (i.e., use the TF-IDF scores to weight the nodes before sum pooling). 
Experiments show that our novel TF-IDF read-out often yields better performance for both models. 

As revealed by the results, GIN constantly fails to distinguish between relevant and irrelevant documents while GAT is relatively better. However, they both fail to improve over the baselines. This is in fact not too surprising considering the actual inductive bias they rely on, which might be unnecessary for document retrieval, and actually make them hard to train and easy to overfit. We defer more in-depth discussion towards this matter into Section \ref{sec:insight}. 

\begin{table}[t]
\centering
% \small
\caption{\label{tab:perform}Model performance on TREC-COVID round 5.}
\resizebox{0.65\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Methods}&\multicolumn{2}{c}{\bf Precision}&\multicolumn{2}{c}{\bf Recall}&\multicolumn{2}{c}{\bf NDCG}\\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
& {\it K=$10$} & {\it K=$20$} & {\it K=$10$} & {\it K=$20$} & {\it K=$10$} & {\it K=$20$} \\
\midrule
{\bf Anserini} & 0.5400 & 0.4960 & 0.0122 & 0.0225 & 0.4709 & 0.4382 \\
{\bf BM25} & 0.5520 & 0.4900 & 0.0136 & 0.0239 & 0.5137 & 0.4591 \\
\midrule
{\bf GIN} & 0.3524 & 0.3436 & 0.0077 & 0.0150 & 0.3059 & 0.2991 \\
{\bf GAT} & 0.4648 & 0.4326 & 0.0108 & 0.0200 & 0.4224 & 0.3949 \\
\midrule 
{\bf N-Pool} & 0.5824 & 0.5220 & 0.0138 & 0.0241 & 0.5338 & 0.4880 \\
\rowcolor{gray!20} {\bf E-Pool} & 0.5960 & 0.5388  & 0.0140 & 0.0249 & 0.5611 & 0.5116 \\
\rowcolor{gray!20} {\bf RW-Pool} &  \bf 0.5984 & \bf 0.5392 &  \bf 0.0142 & \bf 0.0253 & \bf 0.5619 & \bf 0.5141 \\
\bottomrule
\end{tabular}
}
\end{table}
